Feature Statistics Mixing Regularization for Generative Adversarial Networks

In generative adversarial networks, improving discriminators is one of the key components for generation performance. As image classifiers are biased toward texture and debiasing improves accuracy, we investigate 1) if the discriminators are biased, and 2) if debiasing the discriminators will improve generation performance. Indeed, we find empirical evidence that the discriminators are sensitive to the style (e.g., texture and color) of images. As a remedy, we propose feature statistics mixing regularization (FSMR) that encourages the discriminator's prediction to be invariant to the styles of input images. Specifically, we generate a mixed feature of an original and a reference image in the discriminator's feature space and we apply regularization so that the prediction for the mixed feature is consistent with the prediction for the original image. We conduct extensive experiments to demonstrate that our regularization leads to reduced sensitivity to style and consistently improves the performance of various GAN architectures on nine datasets. In addition, adding FSMR to recently-proposed augmentation-based GAN methods further improves image quality. Our code is available at https://github.com/naver-ai/FSMR.

==> Rebuttal_trashbin.tex <==
We thank all reviewers for the valuable comments. We appreciate the positive assessments that the paper is "a" (R1, R2), .... Our contributions are .... We carefully read the comments and address all the concerns. G = generator and D = discriminator for brevity below.
Please note that our method includes not only the feature augmentation, but also consistency loss
for debiasing the Ds.

\underline{\textbf{[cite]}} % Content and Style Disentanglement for Artistic Style Transfer]}
computes distances in ImageNet-pretrained VGG16.


\myparagraph [R2, R5] \textbf{The difference from the related works.}
\textbf{CutMix and Mixup} apply augmentations on images, and it is not done on the feature map like us. \textbf{Manifold-Mixup:} the linear interpolation is performed on the feature map, but the style is not transferred using AdaIN like us. \textbf{StyleMix:} Similar to us, the linear interpolation is used on the feature map and AdaIN technique is also used. However, StyleMix uses an additional extra network when using AdaIN, while we do not need any additional network. \textbf{MoEx}: Reducing style bias requires not only feature statistics mixing (e.g. AdaIN, MoEx, Cutmix, Mixup), but also the consistency loss after feature statistics mixing. MoEx has only the former. \textbf{Our contribution is not feature statistics mixing (e.g. AdaIN, Cutmix, Mixup) itself, but to reduce style bias by applying a consistency loss after feature statistics mixing.} Nevertheless, as R2 suggested, we replace AdaIN in Eq.6 with different augmentations and conduct a comparative experiment. As shown in Table 1, AdaIN shows the best performance compared to the other augmentation methods. FSMR is the reason for its better performance because it imposed consistency loss to reduce the style bias.

Nevertheless, as R2 suggested, we replace AdaIN in Eq.6 with different augmentations and conduct a comparative experiment. As shown in Table 1, AdaIN shows the best performance compared to the other augmentation methods. FSMR is the reason for its better performance because it imposed consistency loss to reduce the style bias.


\myparagraph [R2] \textbf{Comparison to on-the-fly stylization with the internal training images} 
internal 해봤지만 ours보다 구리다. FSMR의 성능향상은 internal보다는.. + adain image 보면 이상하다
% Table에 FSMR 결과까지 넣으면 자리가 좀 필요한데, 어떻게 할까요? jhkim.
As R2 suggested, we conduct an  experiment to the on-the-fly stylization method with the internal training image. As shown in Table 2, Our methods all perform better than the on-the-fly method using external, internal training images and  $^\dagger$ indicates the results of using external training images. Interestingly, using  the external images have better performance than using the internal images. Despite the use of the same data distribution as the training images, the reason why the performance is relatively poor is that the overall structure of the stylized images are not clear and broken when style transferring from the additional extra network as shown in Fig 4. 
% \textbf{Additionally, our method shows that the images are stably regenerated from the mixed feature maps so that we reliably make the discriminator to robust by imposing consistency regularization from this feature maps and the robust discriminator produce the richer gradients to the generator(generate the better samples).}


% While FIDs on MetFaces and AFHQ in ADA are from 1024$\times$1024 and 512$\times$512 resolutions, respectively, our results are from 256$\times$256.
% For MetFaces and AFHQ, the resolution is different(\ie, ADA report FID for 1024$\times$1024 and 512$\times$512, respectively). We all report based on 256$\times$256 resolution.
% \myparagraph [R1] \textbf{The difference in FID from the original paper(ADA)} In short, \textbf{the resolution is different.} In the original paper, ADA, metface and AFHQ-variants reported FID for 1024x1024 and 512x512, respectively. We all report based on 256x256 resolution, so it is different from the FID of the original paper. We used the official code when conducting the experiment, followed the 'paper256' config setting of the code, and did not violate fairness.

% [R1] \textbf{Minor issue} Linear means a fully connected layer to obtain logit. Also, We will add the \textbf{missing word (L842 "using")} after the rebuttal.

%\myparagraph [R2] \textbf{Comparison to existing mixing based data augmentation techniques(Cutmix, Manifold-Mixup)} As suggested, we conduct a comparative experiment by combining each data augmentation techniques with ADA. Please understand that due to the lack of time and resources, we have not been able to experiment with other models and datasets. As shown in Table 1, we can see that our method is superior to the mentioned techniques. Simply using mixing techniques is not our contribution. \textbf{Our contribution is the first to find reducing the style bias in GAN field by applying feature statistics mixing and then imposing consistency regularization loss.}

% \myparagraph [R2] \textbf{Comparison to existing mixing based data augmentation techniques (Cutmix, Manifold-Mixup).} Our contribution is not feature statistics mixing (e.g. AdaIN, Cutmix, Mixup) itself, but to reduce style bias by applying a consistency loss after feature statistics mixing. Nevertheless, as R2 suggested, we replace AdaIN in Eq.6 with different augmentations and conduct a comparative experiment. As shown in Table 1, AdaIN shows the best performance compared to the other augmentation methods.

% \myparagraph [R3] \textbf{Clarify the details of sentences} \textbf{L80-86:} This is a very simple logic. The meaning that "the discriminator is ideal" is the same as that it is not biased toward style. In other words, for example, let's assume that the input images have different styles and same contents. Since the discriminator is ideal that is not biased toward style, it is not affected to the output logit value even if the style is different. Therefore, as a result, the style distance becomes small. \textbf{L105-106:} The mixed feature is the style of reference applied to the source using the AdaIN technique. The regeneration of this as an image is shown in Figure 3 of the original paper. Therefore, if the distance between the logit from the mixed features and the origin logit from the original features(not mixed features) is reduced, it can help to become an ideal discriminator that is not biased toward style as mentioned above. \textbf{L119:} Yes. This sentence is a complete sentence. We accidentally missed the period. \textbf{L221:} We think it probably means L121. Since this is a bullet description of the contribution point, Section 2 is mentioned without describing the details. \textbf{L2, L367-369:} We have described several times in Section 2 what style bias is, content distance, style distance, and relative distance. In addition, what our method FSMR is and how this style bias is solved have been described several times in Section 3 and 4.

\myparagraph [R4] \textbf{How to explain the smaller relative distance indeed corresponds to better generated image quality?} \textbf{This is a very simple logic.} It is well known that reducing style bias in the field of classification will robust the network and improve classification performance. In GANs, since the generator and the discriminator are trained adversarially with each other, the robuster the discriminator, the better the performance (generative quality) of the generator. Since the discriminator is a classifier that classifies real and fake, if we show that the discriminator also has a style bias, we can try to improve performance by making the discriminator robuster by mitigating it. So we proposed the relative distance to prove that the discriminator also has a style bias. Therefore, in summary, if the relative distance associated with the degree of style bias becomes smaller, the discriminator becomes robuster, and as a result, the performance of the generator increases. Therefore, it can be said that the relative distance is related to the generated image quality.

\myparagraph [R4] \textbf{Clarify the Figiure 4} \textbf{It's not contradictory.} The degree of style bias of the network varies depending on the augmentation or regularization. Therefore, the relative distance representing style bias is not used to compare between different models, but a method for comparing between the same models. 


\myparagraph [R4] \textbf{Clarify the Table 3,4} \textbf{CIFAR10:} When measuring the FID, we followed the FID measurement method in the original ADA code. In the case of StyleGAN2 FID you mentioned, the official code implemented inside the ADA was also used as it is. The reason why StyleGAN2's FID was low at 3.89 is presumed to be because the official implementation code (StyleGAN2 inside the ADA) was slightly different compared to the original StyleGAN2 code. (For example, it is described in github that the number of mapping layers in genertor changes from 8 to 2, and is set to a better hyperparameter setting.) \textbf{DiffAug:} DiffAug's FID measurement method and ADA's FID measurement method are completely different. DiffAug measures FID with (10k) validation images, and ADA measures FID with (50k) training images. Therefore, when measuring the FID, the number of images and the types of images are different, so it is different from the FID of the original DiffAug paper, and we followed the FID measurement method of ADA. The best FID was the same, but the standard deviation was different. \textbf{Cifar10 with unconditional and conditional settings:} When we checked, there were some typos. For example, in the case of conditional setting of StyleGAN2, it was accidentally reported as an unconditional settings value. This value will be revised to 3.87 $\rightarrow$  3.52, and in the case of DiffAug with FSMR, it will be revised to 2.97 $\rightarrow$ 2.87.


\myparagraph [R5] \textbf{Technical novelty is limited. FSMR is very similar to MoEx.} Our contribution is not feature statisics mixing (e.g. AdaIN, MoEx, Cutmix, Mixup) itself, but to reduce style bias by applying a consistency loss after feature statistics mixing. In addition, MoEx itself is the same as AdaIN operation. %yjc: 마지막 문장은 필요없다 생각하면 지우셔도 됩니다.

